SoK: A Systems Perspective on Compound AI Threats and Countermeasures

Large language models (LLMs) used across enterprises often use proprietary models and operate on sensitive inputs and data. The wide range of attack vectors identified in prior research - targeting various software and hardware components used in training and inference - makes it extremely challenging to enforce confidentiality and integrity policies. As we advance towards constructing compound AI inference pipelines that integrate multiple large language models (LLMs), the attack surfaces expand significantly. Attackers now focus on the AI algorithms as well as the software and hardware components associated with these systems. While current research often examines these elements in isolation, we find that combining cross-layer attack observations can enable powerful end-to-end attacks with minimal assumptions about the threat model. Given, the sheer number of existing attacks at each layer, we need a holistic and systemized understanding of different attack vectors at each layer. This SoK discusses different software and hardware attacks applicable to compound AI systems and demonstrates how combining multiple attack mechanisms can reduce the threat model assumptions required for an isolated attack. Next, we systematize the ML attacks in lines with the Mitre Att&ck framework to better position each attack based on the threat model. Finally, we outline the existing countermeasures for both software and hardware layers and discuss the necessity of a comprehensive defense strategy to enable the secure and high-performance deployment of compound AI systems.

==> content/criticality.tex <==
\section{Criticality of attacks and defenses:}

%   Enlist the criticality of each attacks --- Maybe a table
%   Enlist the criticality of defenses --  Argue with the defense overhead -- perf, traffic, power, area
% Chronology of each attack surface 
% Back of envelope calculation of defence overhead 
This section is dedicated 

\begin{itemize}
    \item Latest and greatest attacks
    \item Having high level attacker does not require a lot of privileges
    \item Remote attacker
    \item Map attacks with varying attacker capability 
    \item New metrics -- Ease, capability, severity
    \item View from defense perspective 
    \item Hardware attack metrics --- Rank attacks based on leakage (Netspectre)
    \item Simha's side-channel metric (e.g.,<bits/sec>https://www.cs.columbia.edu/~simha/preprint\_isca12\_svf.pdf)
    \item Observability
    \item Model owner, CSP, data owner, Other tenants
    \item \anjo{Attacks earlier in the compound AI system are more critical}
    \item \anjo{security policies and privacy is achieved throughout the system and not by a single entity}
    \item \anjo{complex HW/SW stack with lots of dependencies}
    \item \anjo{learnings? targets to secure? can we identify things that are particularly error prone and important?}
\end{itemize}
